Pointer-Chase Prefetcher for Linked Data Structures

Caches only exploit spatial and temporal locality in a set of address referenced in a program. Due to dynamic construction of linked data-structures, they are difficult to cache as the spatial locality between the nodes is highly dependent on the data layout. Prefetching can play an important role in improving the performance of linked data-structures. In this project, a pointer chase mechanism along with compiler hints is adopted to design a prefetcher for linked data-structures. The design is evaluated against the baseline of processor with cache in terms of performance, area and energy

==> Makefile <==
OBJ = obj
LATEX = pdflatex -output-directory $(OBJ)
BIBTEX = bibtex
DVIPS = dvips
PS2PDF = ps2pdf

MAIN_DOC = main

all:
	mkdir -p $(OBJ);
	$(LATEX) $(MAIN_DOC).tex;
	$(BIBTEX) $(OBJ)/$(MAIN_DOC); 
	$(LATEX) $(MAIN_DOC).tex;
	$(LATEX) $(MAIN_DOC).tex;
	cp $(OBJ)/$(MAIN_DOC).pdf .

tar:
	rm -f $(MAIN_DOC).tar.gz $(MAIN_DOC).tar; tar -cf $(MAIN_DOC).tar *.sty *.tex *.bib makefile $(MAIN_DOC).ps.gz EPS/*.eps TAB/*.tex outline; gzip $(MAIN_DOC).tar;


clean:
	rm -rf   \
                *.aux \
                *.lot \
                *.lof \
                *.bbl \
                *.toc \
                *.blg \
                *.dvi \
                *.log \
                *.out \
                *.ps  \
                *~ \
                BIB/*~ \
                $(OBJ)


